Blue noise for diffusion models

Most of the existing diffusion models use Gaussian noise for training and sampling across all time steps, which may not optimally account for the frequency contents reconstructed by the denoising network. Despite the diverse applications of correlated noise in computer graphics, its potential for improving the training process has been underexplored. In this paper, we introduce a novel and general class of diffusion models taking correlated noise within and across images into account. More specifically, we propose a time-varying noise model to incorporate correlated noise into the training process, as well as a method for fast generation of correlated noise mask. Our model is built upon deterministic diffusion models and utilizes blue noise to help improve the generation quality compared to using Gaussian white (random) noise only. Further, our framework allows introducing correlation across images within a single mini-batch to improve gradient flow. We perform both qualitative and quantitative evaluations on a variety of datasets using our method, achieving improvements on different tasks over existing deterministic diffusion models in terms of FID metric.

==> figures/3-axis_visualization/3-axis_visualization.tex <==
%!TEX root = ../paper.tex

\newcommand{\PlotSingleImage}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/3-axis_visualization/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
    % \end{tikzpicture}%
}

\newcommand{\TwoColumnFigure}[2]{%
    \begin{tabular}{c@{\;}c@{}}
        \hspace*{-2.5mm}
        \begin{tikzpicture}[scale=0.535]    % 0.565
            \PlotSingleImage{#1}
        \end{tikzpicture}
         & 
         \begin{tikzpicture}[scale=0.535]
            \PlotSingleImage{#2}
        \end{tikzpicture}
    \end{tabular}%
}

\newcommand{\scaleval}{1.1} % 1.16
\small
\hspace*{-4mm}
\begin{tabular}{c@{\;}c@{\;}c@{\;}c@{}}
%
~ &
Random &
Correlated data &
Correlated data \& content
\\
\rotatebox{90}{\hspace{0.5cm} \scriptsize Data distribution}
&
\begin{tikzpicture}[scale=\scaleval]
    \PlotSingleImage{logo_WN.png}
    \begin{scope}
        \draw [blue,-{Stealth[width=2mm]}](0.69,1.8) -- (0.5,-0.1); % 0.0
        \draw [blue,-{Stealth[width=2mm]}](1.77,0.7) -- (2.0,-0.1);
    \end{scope}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
    \PlotSingleImage{logo_BN.png}
    \begin{scope}
        \draw [blue,-{Stealth[width=2mm]}](0.7,1.7) -- (0.5, -0.1);
        \draw [blue,-{Stealth[width=2mm]}](1.87,0.7) -- (2.0, -0.1);
    \end{scope}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
    \PlotSingleImage{logo_BN.png}
    \begin{scope}
        \draw [blue,-{Stealth[width=2mm]}](0.7,1.7) -- (0.5, -0.1);
        \draw [blue,-{Stealth[width=2mm]}](1.87,0.7) -- (2.0, -0.1);
    \end{scope}
\end{tikzpicture}
\\[-0.4mm]
\rotatebox{90}{\hspace{-0.5cm} \scriptsize Data content}
&
\TwoColumnFigure{cat_res128_00005_wn.png}{cat_res128_00014_wn.png}
&
\TwoColumnFigure{cat_res128_00018_wn.png}{cat_res128_00019_wn.png}
&
\TwoColumnFigure{cat_res128_00018_bn.png}{cat_res128_00019_bn.png}
\end{tabular}


==> figures/3-axis_visualization/Correlated_data.tex <==
%!TEX root = ../paper.tex

\newcommand{\PlotSingleImage}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/3-axis_visualization/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
    % \end{tikzpicture}%
}
\newcommand{\PlotSingleImageBlue}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/3-axis_visualization/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw [blue] (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
    % \end{tikzpicture}%
}
\newcommand{\PlotSingleImageRed}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/3-axis_visualization/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw [red] (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
    % \end{tikzpicture}%
}


\newcommand{\TwoColumnFigure}[2]{%
    \begin{tabular}{c@{\;}c@{}}
        \hspace*{-2.5mm}
        \begin{tikzpicture}[scale=0.535]    % 0.565
            \PlotSingleImageBlue{#1}
        \end{tikzpicture}
         & 
         \begin{tikzpicture}[scale=0.535]
            \PlotSingleImageRed{#2}
        \end{tikzpicture}
    \end{tabular}%
}

\newcommand{\scaleval}{1.1} % 1.16
\small
\hspace*{-4mm}
\begin{tabular}{c@{\;}c@{\;}c@{\;}c@{}}
%
~ &
Gaussian noise &
Gaussian blue noise &
\begin{tabular}{c@{}}
Gaussian blue noise\\
+ Data correlation
\end{tabular}
\\
\rotatebox{90}{\hspace{0.6cm} \scriptsize Data distribution}
&
\begin{tikzpicture}[scale=\scaleval]    
     \PlotSingleImage{diffusion_distribution.png}
     \PlotSingleImage{diffusion_points_bis.png}
    \begin{scope}
        \draw [blue,-{Stealth[width=2mm]}](0.45,1.58) -- (0.5,-0.1); % 0.0
        \draw [red,-{Stealth[width=2mm]}](2.005,0.25) -- (2.0,-0.1);
    \end{scope}
\end{tikzpicture}
%\begin{tikzpicture}[scale=\scaleval]
%    \PlotSingleImage{logo_WN.png}
%    \begin{scope}
%        \draw [blue,-{Stealth[width=2mm]}](0.69,1.8) -- (0.5,-0.1); % 0.0
%        \draw [blue,-{Stealth[width=2mm]}](1.77,0.7) -- (2.0,-0.1);
%    \end{scope}
%\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
    %\PlotSingleImage{logo_BN.png}
    \PlotSingleImage{diffusion_distribution.png}
    \PlotSingleImage{diffusion_points.png}
    \begin{scope}
        \draw [blue,-{Stealth[width=2mm]}](0.275,1.76) -- (0.5,-0.1); % 0.0
        \draw [red,-{Stealth[width=2mm]}](2.005,0.25) -- (2.0,-0.1);
    \end{scope}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
    %\PlotSingleImage{logo_BN.png}
    \PlotSingleImage{diffusion_distribution.png}
    \PlotSingleImage{diffusion_points_remap.png}
    \begin{scope}
        \draw [blue,-{Stealth[width=2mm]}](0.275,1.76) -- (0.5,-0.1); % 0.0
        \draw [red,-{Stealth[width=2mm]}](2.005,0.25) -- (2.0,-0.1);
    \end{scope}
\end{tikzpicture}
\\[-0.4mm]
\rotatebox{90}{\hspace{-0.5cm} \scriptsize Data content}
&
\TwoColumnFigure{wn_res64.png}{0000169.png}%{cat_res128_00014_wn.png}
&
\TwoColumnFigure{bn_res64.png}{0000169.png}%{cat_res128_00019_wn.png}
&
\TwoColumnFigure{bn_res64.png}{0000169.png}%{cat_res128_00019_bn.png}
\\
~ & (a) & (b) & (c)
\end{tabular}


==> figures/teaser/teaser_v0.tex <==
%!TEX root = ../paper.tex

\newcommand{\PlotSingleImage}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
    % \end{tikzpicture}%
}


\newcommand{\PlotSingleImageWithLine}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
         \draw[dashed] (0, -0.13) -- (2.5, -0.13);
    % \end{tikzpicture}%
}



\newcommand{\TwoColumnFigure}[2]{%
    \begin{tabular}{c@{\;}c@{}}
        \hspace*{-2.5mm}
        \begin{tikzpicture}[scale=0.563]
            \PlotSingleImage{#1}
        \end{tikzpicture}
         & 
         \begin{tikzpicture}[scale=0.563]
            \PlotSingleImage{#2}
        \end{tikzpicture}
    \end{tabular}%
}

\newcommand{\scaleval}{0.67}

\small
\hspace*{-4mm}
\begin{tabular}{c@{\;}c@{\;}c@{\;}c@{\;}c@{\;}c@{\;}c@{\;}c@{\;}c@{\;}c@{\;}c@{}}
%
% ~ &
% $t=999$ & 
% $t=800$ &
% $t=700$ &
% $t=600$ &
% $t=500$ &
% $t=400$ &
% $t=300$ &
% $t=200$ &
% $t=100$ &
% $t=0$
% \\
\rotatebox{90}{\scriptsize \; \, Random noise}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step0.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step25.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step50.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step100.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step125.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step150.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step175.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step200.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step225.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step250.png}
\end{tikzpicture}
%%%%%%%%%%%%%%%%%%%%%%%%%
\\[-0.4mm]
%%%%%%%%%%%%%%%%%%%%%%%%%
\rotatebox{90}{\scriptsize \; Blue noise (Ours)}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step0.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step25.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step50.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step100.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step125.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step150.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step175.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step200.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step225.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step250.png}
\end{tikzpicture}
%%%%%%%%%%%%%%%%%%%%%%%%%
\\[-0.4mm]
%%%%%%%%%%%%%%%%%%%%%%%%%
\rotatebox{90}{\scriptsize Time-varying (Ours)}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step0.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step25.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step50.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step100.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step125.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step150.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step175.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step200.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step225.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step250.png}
\end{tikzpicture}
%%%%%%%%%%%%%%%%%%%%%%%%%
\\[-0.4mm]
%%%%%%%%%%%%%%%%%%%%%%%%%
\rotatebox{90}{\scriptsize \; Our noise masks}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t250.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t225.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t200.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t150.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t125.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t100.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t075.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t050}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t025}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t000}
\end{tikzpicture}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\[-0.4mm]
%%%%%%%%%%%%%%%%%%%%%%%%%%%
~ &
$t=250$ & 
$t=225$ &
$t=200$ &
$t=150$ &
$t=125$ &
$t=100$ &
$t=75$ &
$t=50$ &
$t=25$ &
$t=0$
\end{tabular}


==> figures/teaser/teaser_v1.tex <==
%!TEX root = ../paper.tex

\newcommand{\PlotSingleImage}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
    % \end{tikzpicture}%
}


\newcommand{\PlotSingleImageWithLine}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
         \draw[dashed] (0, -0.13) -- (2.5, -0.13);
    % \end{tikzpicture}%
}



\newcommand{\TwoColumnFigure}[2]{%
    \begin{tabular}{c@{\;}c@{}}
        \hspace*{-2.5mm}
        \begin{tikzpicture}[scale=0.563]
            \PlotSingleImage{#1}
        \end{tikzpicture}
         & 
         \begin{tikzpicture}[scale=0.563]
            \PlotSingleImage{#2}
        \end{tikzpicture}
    \end{tabular}%
}

\newcommand{\mycomment}[1]{#1}
%\newcommand{\scaleval}{0.67}
\newcommand{\scaleval}{0.7}
\newcommand{\scalevalShortcut}{0.7}

\small
\hspace*{-4mm}
\begin{tabular}{p{0.75\textwidth}p{0.25\textwidth}}
\begin{tabular}{c@{\;}c@{\;}c@{\;}c@{\;}c@{\;}c@{\;}c@{\;}c@{}}
%
% ~ &
% $t=999$ & 
% $t=800$ &
% $t=700$ &
% $t=600$ &
% $t=500$ &
% $t=400$ &
% $t=300$ &
% $t=200$ &
% $t=100$ &
% $t=0$
% \\
\rotatebox{90}{\scriptsize \; \, \cite{heitz2023iterative}}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step0.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step50.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step125.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step175.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step200.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step225.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step250.png}
\end{tikzpicture}
%%%%%%%%%%%%%%%%%%%%%%%%%
\\[-0.4mm]
%%%%%%%%%%%%%%%%%%%%%%%%%
\rotatebox{90}{\scriptsize \; Blue noise (Ours)}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step0.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step50.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step125.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step175.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step200.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step225.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step250.png}
\end{tikzpicture}
%\mycomment{
%%%%%%%%%%%%%%%%%%%%%%%%%
\\[-0.4mm]
%%%%%%%%%%%%%%%%%%%%%%%%%
\rotatebox{90}{\scriptsize Time-varying (Ours)}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step0.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step50.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step125.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step175.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step200.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step225.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step250.png}
\end{tikzpicture}
%}
%%%%%%%%%%%%%%%%%%%%%%%%%
\\[-0.4mm]
%%%%%%%%%%%%%%%%%%%%%%%%%
\rotatebox{90}{\scriptsize \; Our noise masks}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t250.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t200.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t125.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t075.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t050.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t025.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t000.png}
\end{tikzpicture}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\[-0.4mm]
%%%%%%%%%%%%%%%%%%%%%%%%%%%
~ &
$t=250$ & 
$t=200$ &
$t=125$ &
$t=75$ &
$t=50$ &
$t=25$ &
$t=0$
\end{tabular}
&

\begin{tabular}{c@{\;}c@{\;}c@{}}

\rotatebox{90}{\large \; \hspace{0.3cm} 30\%}
&
\begin{tikzpicture}[scale=\scalevalShortcut]
\PlotSingleImage{celeba_res64_shortcut_diffusion/gaussian_alpha0.30_img00000.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalShortcut]
\PlotSingleImage{celeba_res64_shortcut_diffusion/gaussianBN_alpha0.30_img00000.png}
\end{tikzpicture}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\[-0.4mm]
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rotatebox{90}{\large \; \hspace{0.3cm} 50\%}
&
\begin{tikzpicture}[scale=\scalevalShortcut]
\PlotSingleImage{celeba_res64_shortcut_diffusion/gaussian_alpha0.50_img00000.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalShortcut]
\PlotSingleImage{celeba_res64_shortcut_diffusion/gaussianBN_alpha0.50_img00000.png}
\end{tikzpicture}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\[-0.4mm]
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rotatebox{90}{\large \; \hspace{0.3cm} 70\%}
&
\begin{tikzpicture}[scale=\scalevalShortcut]
\PlotSingleImageWithLine{celeba_res64_shortcut_diffusion/gaussian_alpha0.70_img00000.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalShortcut]
\PlotSingleImageWithLine{celeba_res64_shortcut_diffusion/gaussianBN_alpha0.70_img00000.png}
\end{tikzpicture}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\[-0.4mm]
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rotatebox{90}{\large \; Reference}
&
\begin{tikzpicture}[scale=\scalevalShortcut]
\PlotSingleImage{celeba_res64_shortcut_diffusion/0025001.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalShortcut]
\PlotSingleImage{celeba_res64_shortcut_diffusion/0025001.png}
\end{tikzpicture}\\

~ &
\small \cite{heitz2023iterative} & 
\large \textbf{Ours}


\end{tabular}

\end{tabular}

==> figures/teaser/teaser_v2.tex <==
%!TEX root = ../paper.tex

\newcommand{\PlotSingleImage}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
    % \end{tikzpicture}%
}


\newcommand{\PlotSingleImageWithLine}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
         \draw[dashed] (0, -0.13) -- (2.5, -0.13);
    % \end{tikzpicture}%
}



\newcommand{\TwoColumnFigure}[2]{%
    \begin{tabular}{c@{\;}c@{}}
        \hspace*{-2.5mm}
        \begin{tikzpicture}[scale=0.563]
            \PlotSingleImage{#1}
        \end{tikzpicture}
         & 
         \begin{tikzpicture}[scale=0.563]
            \PlotSingleImage{#2}
        \end{tikzpicture}
    \end{tabular}%
}

\newcommand{\mycomment}[1]{#1}
%\newcommand{\scaleval}{0.67}
\newcommand{\scaleval}{0.72}
\newcommand{\scalevalShortcut}{0.729}

\small
\hspace*{-4mm}
\begin{tabular}{p{0.755\textwidth}p{0.16\textwidth}}
\begin{tabular}{c@{\;}c@{\;}c@{\;}c@{\;}c@{\;}c@{\;}c@{\;}c@{}}
%
% ~ &
% $t=999$ & 
% $t=800$ &
% $t=700$ &
% $t=600$ &
% $t=500$ &
% $t=400$ &
% $t=300$ &
% $t=200$ &
% $t=100$ &
% $t=0$
% \\
\rotatebox{90}{\hspace{0.15cm}\scriptsize \citet{heitz2023iterative}}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step0.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step50.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step125.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step175.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step200.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step225.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gwn_img02000_step250.png}
\end{tikzpicture}
%%%%%%%%%%%%%%%%%%%%%%%%%
\\[-0.4mm]
%%%%%%%%%%%%%%%%%%%%%%%%%
\rotatebox{90}{\hspace{0.1cm} \scriptsize Blue noise (Ours)}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step0.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step50.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step125.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step175.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step200.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step225.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{cat_res128_iadb/gbn_img00000_step250.png}
\end{tikzpicture}
%\mycomment{
%%%%%%%%%%%%%%%%%%%%%%%%%
\\[-0.4mm]
%%%%%%%%%%%%%%%%%%%%%%%%%
\rotatebox{90}{\hspace{0.1cm}\scriptsize Time-varying (Ours)}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step0.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step50.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step125.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step175.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step200.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step225.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImageWithLine{cat_res128_iadb_linear_teaser/gwn2gbn_img02000_step250.png}
\end{tikzpicture}
%}
%%%%%%%%%%%%%%%%%%%%%%%%%
\\[-0.4mm]
%%%%%%%%%%%%%%%%%%%%%%%%%
\rotatebox{90}{\hspace{0.2cm}\scriptsize Our noise masks}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t250.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t200.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t125.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t075.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t050.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t025.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scaleval]
\PlotSingleImage{interpolated_noises_res128/interpolated_noise_t000.png}
\end{tikzpicture}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\[-0.4mm]
%%%%%%%%%%%%%%%%%%%%%%%%%%%
~ &
$t=250$ & 
$t=200$ &
$t=125$ &
$t=75$ &
$t=50$ &
$t=25$ &
$t=0$
\end{tabular}
&
\vline width 1.5pt
\begin{tabular}{c@{\;}c@{\;}c@{}}

% \rotatebox{90}{\large \; \hspace{0.3cm} 30\%}
&
\begin{tikzpicture}[scale=\scalevalShortcut]
\PlotSingleImage{teaser/gwn_img18000_step250.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalShortcut]
\PlotSingleImage{teaser/gwn2gbn_img18000_step250.png}
\end{tikzpicture}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\[-0.4mm]
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \rotatebox{90}{\large \; \hspace{0.3cm} 50\%}
&
\begin{tikzpicture}[scale=\scalevalShortcut]
\PlotSingleImage{teaser/gwn_img16000_step250.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalShortcut]
\PlotSingleImage{teaser/gwn2gbn_img16000_step250.png}
\end{tikzpicture}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\[-0.4mm]
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \rotatebox{90}{\large \; \hspace{0.3cm} 70\%}
&
\begin{tikzpicture}[scale=\scalevalShortcut]
\PlotSingleImage{teaser/gwn_img05200_step250.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalShortcut]
\PlotSingleImage{teaser/gwn2gbn_img05200_step250.png}
\end{tikzpicture}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\[-0.4mm]
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \rotatebox{90}{\large \; Reference}
&
\begin{tikzpicture}[scale=\scalevalShortcut]
\PlotSingleImage{teaser/gwn_img00000_step250.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalShortcut]
\PlotSingleImage{teaser/gwn2gbn_img00000_step250.png}
\end{tikzpicture}\\

~ &
\footnotesize \citet{heitz2023iterative} & 
\large \textbf{Ours}


\end{tabular}

\end{tabular}


